Search for microscopic black holes and string balls in final states with leptons and jets with the ATLAS detector at sqrt(s) = 8 TeV

A search for an excess of events with multiple high transverse momentum objects including charged leptons and jets is presented, using 20.3 fb^-1 of proton-proton collision data recorded by the ATLAS detector at the Large Hadron Collider in 2012 at a centre-of-mass energy of sqrt(s) = 8 TeV. No excess of events beyond Standard Model expectations is observed. Using extra-dimensional models for black hole and string ball production and decay, exclusion contours are determined as a function of the mass threshold for production and the fundamental gravity scale for two, four and six extra dimensions. For six extra dimensions, mass thresholds of 4.8-6.2 TeV are excluded at 95% confidence level, depending on the fundamental gravity scale and model assumptions. Upper limits on the fiducial cross-sections for non-Standard Model production of these final states are set.

==> cutflowTables.tex <==
\begin{table*}[htb]
	\footnotesize
	\begin{center}
		\begin{tabular}{|c|c|}%{\textwidth}@{\extracolsep{\fill}
			\hline
			\textbf{Requirement}  & \textbf{Number of Events passing} \\  \hline
			Initial & 10000 \\  \hline
			Trigger     &     2297 \\  \hline
			Primary Vertex   &   2294 \\  \hline
			Jet Cleaning &  2273 \\ \hline
			One lepton above 60 \GeV &      915 \\ \hline
			Trigger matching &     909 \\ \hline
			Three Objects above 60 \GeV  &    879 \\ \hline
			Three Objects above 100 \GeV  &    848 \\ \hline
			$\sumpt > 3000~\GeV$ & 685 \\ \hline
			
		\end{tabular}
	\end{center}
	\caption{Cut-flow for a signal point in the rotating BH model with $n=6$, \MTH = 6 \TeV~and \MD = 4 \TeV, simulated with \charybdis. The cross-section calculated by \charybdis is $0.0911$ pb.}
	\label{tab:cutflowOne}
\end{table*}

%/mc12_8TeV.159428.Charybdis2Pythia8_AU2MSTW2008LO_BH2_n6_Mth6_0_MD4_0.merge.NTUP_SUSY.e1649_a159_a171_r3549_p1328_tid01137108_00


\begin{table*}[htb]
	\footnotesize
	\begin{center}
		\begin{tabular}{|c|c|}%{\textwidth}@{\extracolsep{\fill}
			\hline
			\textbf{Requirement}  & \textbf{Number of Events passing} \\  \hline
			Initial & 10000 \\  \hline
			Trigger     &     2340 \\  \hline
			Primary Vertex   &   2316  \\  \hline
			Jet Cleaning &  2294 \\ \hline
			One lepton above 60 \GeV &      990 \\ \hline
			Trigger matching &     975 \\ \hline
			Three Objects above 60 \GeV  &    954 \\ \hline
			Three Objects above 100 \GeV  &    945 \\ \hline
			$\sumpt > 3000~\GeV$ & 709 \\ \hline
		\end{tabular}
	\end{center}
	\caption{Cut-flow for a signal point in the rotating BH model with $n=6$, \MTH = 5.5 \TeV~and \MD = 3 \TeV, simulated with \charybdis. The cross-section calculated by \charybdis is $2.21$ pb.}
	\label{tab:cutflowTwo}
\end{table*}
%mc12_8TeV.159420.Charybdis2Pythia8_AU2MSTW2008LO_BH2_n6_Mth5_5_MD3_0.merge.NTUP_SUSY.e1649_a159_a171_r3549_p1328_tid01137100_00:

